KARLA: Knowledge-base Augmented Retrieval for Language Models

We propose a new method that allows an LLM to automatically pull in factual knowledge from a knowledge base during token generation. This means that (1)~factual knowledge in the LLM output can be updated without retraining the LLM, (2)~facts in the LLM output can be traced to the knowledge base for transparency and explainability, and (3)~smaller models can achieve the same factual accuracy as larger models. Our core idea is to train the model to produce special tokens that trigger a query to the knowledge base. Our experiments show that our method improves factual grounding in both short and long-form generation, and allows factual revisions to take effect through KB edits rather than parameter updates.

==> figures/KARLA_in_action.tex <==

\begin{tikzpicture}[
  font=\small,
  special/.style={
    rectangle, rounded corners=1.5pt, draw=purple!70!black, fill=purple!12,
    text=purple!45!black, font=\tiny\ttfamily, inner sep=1.5pt, minimum height=3.6mm
  },
  subj/.style={
    rectangle, rounded corners=1.5pt, draw=teal!70!black, fill=teal!15,
    text=teal!40!black, font=\tiny\ttfamily, inner sep=1.5pt, minimum height=3.6mm
  },
  kbval/.style={
    rectangle, rounded corners=1.5pt, draw=orange!80!black, fill=orange!22,
    text=orange!50!black, font=\tiny\ttfamily, inner sep=1.5pt, minimum height=3.6mm
  },
  plain/.style={
    rectangle, rounded corners=1.5pt, draw=gray!50, fill=gray!10,
    text=black, font=\tiny, inner sep=1.5pt, minimum height=3.6mm
  },
  promptbox/.style={
    rectangle, rounded corners=2pt, draw=gray!60!black, fill=gray!8,
    text=black, font=\tiny\itshape, inner sep=3pt, align=center
  },
  llmbox/.style={
    rectangle, rounded corners=2.5pt, draw=blue!60!black, fill=blue!10,
    text=blue!45!black, font=\tiny\bfseries, inner sep=2.5pt,
    minimum width=15mm, minimum height=7mm, align=center
  },
  flow/.style={->, >=Stealth, semithick, gray!55!black},
  flowR/.style={->, >=Stealth, semithick, orange!65!black},
  flowL/.style={->, >=Stealth, semithick, blue!55!black},
  legendbox/.style={rectangle, rounded corners=1pt, minimum width=2mm, minimum height=2mm, draw, inner sep=0pt},
]

% --- 1. Prompt (top) ---
\node[promptbox] (prompt) at (0,0)
  {Prompt: ``Paris has a population of''};

% --- 2. KARLA below the prompt ---
\node[llmbox, below=2.5mm of prompt] (llm) {KARLA\\\tiny\mdseries (fine-tuned LM)};
\draw[flowL] (prompt.south) -- (llm.north);

% --- 3. KB cylinder on the right ---
\coordinate (kbcenter) at ($(llm.east) + (1.85, 0.30)$);
\begin{scope}[shift={(kbcenter)}]
  \filldraw[fill=orange!12, draw=orange!75!black, semithick]
    (-0.7, 0) -- (-0.7, -0.7)
    arc[start angle=180, end angle=360, x radius=0.7, y radius=0.17]
    -- (0.7, 0)
    arc[start angle=0, end angle=180, x radius=0.7, y radius=0.17];
  \filldraw[fill=orange!22, draw=orange!75!black, semithick]
    (0, 0) ellipse[x radius=0.7, y radius=0.17];
  \draw[orange!55!black, dashed, thin]
    (-0.7, 0) arc[start angle=180, end angle=0, x radius=0.7, y radius=0.17];
  \node[font=\tiny\bfseries, text=orange!50!black] at (0, -0.40) {Knowledge};
  \node[font=\tiny\bfseries, text=orange!50!black] at (0, -0.60) {base};
\end{scope}
\coordinate (kbBottomMid) at ($(kbcenter) + (0, -0.87)$);

% --- 5. Generated token stream ---
% Position t1 so that its TOP-LEFT sits directly under llm.south,
% giving us a clean vertical "generates" arrow.
\node[special, anchor=north west] (t1) at ($(llm.south) + (-0.50, -1.20)$)
  {$\langle$populationTotal$\rangle$};
\node[special, right=0.4mm of t1] (t2) {$\langle$subj$\rangle$};
\node[subj,    right=0.4mm of t2] (t3) {Paris};
\node[special, right=0.4mm of t3] (t4) {$\langle$/subj$\rangle$};

\node[special, below=3.5mm of t1.south west, anchor=north west] (t5)
  {$\langle$KB$\rangle$};
\node[kbval,   right=0.4mm of t5] (t6) {2{,}102{,}650};
\node[special, right=0.4mm of t6] (t7) {$\langle$/KB$\rangle$};
\node[plain,   right=0.4mm of t7] (t8) {2{,}102{,}650 inhabitants \ldots};

% --- 5a. Tinted background marking the model-GENERATED tokens ---
% Generated: row A entirely (t1..t4) + tail of row B (t8).
% NOT generated: the <KB> o </KB> block (t5..t7) — filled by the executor.
%
% We draw two soft rounded rectangles in the background layer:
%   (i)  around row A (t1..t4)
%   (ii) around t8 only on row B
\begin{scope}[on background layer]
  % Row A background
  \node[fit=(t1)(t4), rounded corners=3pt,
        fill=blue!6, draw=blue!35, thin,
        inner sep=1.5pt] (genA) {};
  % Row B tail (t8 only)
  \node[fit=(t8), rounded corners=3pt,
        fill=blue!6, draw=blue!35, thin,
        inner sep=1.5pt] (genB) {};
\end{scope}

% (no separate text label: the blue tint + "generates" arrow + legend swatch
%  below convey that this is the model-generated region.)

% (the orange tokens + orange "returns value" arrow already mark this
%  span as KB-filled; no extra brace needed.)

% --- 6. KARLA -> token stream "generates" arrow (STRAIGHT, vertical) ---
\draw[flowL] (llm.south) -- ($(llm.south |- genA.north) + (0, 0.02)$);
\node[font=\tiny\itshape, text=blue!45!black, anchor=east, inner sep=1pt]
  at ($(llm.south)!0.5!(llm.south |- genA.north) + (-0.04, 0)$) {generates};

% --- 4. QUERY arrow: from <populationTotal> (relation) + Paris (subject) ---
\coordinate (qRelTop)  at (t1.north);
\coordinate (qSubTop)  at (t3.north);
\coordinate (qLaneY)   at ($(genA.north) + (0, 0.30)$);
\coordinate (qRelLane) at (t1.north |- qLaneY);
\coordinate (qSubLane) at (t3.north |- qLaneY);

\draw[semithick, gray!55!black, rounded corners=2pt]
  (qRelTop) -- (qRelLane);
\draw[semithick, gray!55!black, rounded corners=2pt]
  (qSubTop) -- (qSubLane);

\draw[flow, rounded corners=2pt]
  (qRelLane) -- (qSubLane) -- (kbBottomMid |- qSubLane) -- (kbBottomMid);

% (no merge dot at the junction)

% "query" label: place on the horizontal segment, anchored east of the corner
% (i.e. to the left of the vertical riser), so it does not overlap the arrow.
\node[font=\tiny, text=gray!40!black, anchor=east]
  at ($(kbBottomMid |- qSubLane) + (-0.15, 0.10)$) {query};

% --- 7. Return arrow: KB -> KB-value token in row B ---
\coordinate (kbExit)    at ($(kbcenter) + (0.5, -0.78)$);
\coordinate (rightCol)  at ($(t8.east)   + (0.30, 0)$);
\coordinate (laneY)     at ($(t5.south)  + (0, -0.45)$);

\coordinate (rTopRight) at (rightCol |- kbExit);
\coordinate (rBotRight) at (rightCol |- laneY);
\coordinate (rBotLeft)  at (t6.south  |- laneY);

\draw[flowR, rounded corners=2pt]
  (kbExit) -- (rTopRight) -- (rBotRight) -- (rBotLeft) -- (t6.south);
\node[font=\tiny, text=orange!55!black, anchor=north]
  at ($(rBotLeft)!0.5!(rBotRight) + (0, -0.02)$) {returns value};

% --- 8. Legend (centered horizontally below the figure) ---
% Compute the figure's horizontal center from its actual extents:
% leftmost point  = prompt's left edge
% rightmost point = the return arrow's right column (just past t8)
\coordinate (figCenter) at ($(prompt.west)!0.5!(rightCol)$);

% Build the legend as a single group of nodes anchored to a central point.
\node[anchor=center, inner sep=0pt]
  (legend) at ($(figCenter) + (0, -2.75)$)
  {%
    \tikz[baseline]{%
      \node[legendbox, draw=blue!35, fill=blue!6, anchor=west] (lgen) at (0,0) {};
      \node[right=0.6mm of lgen, font=\tiny] (lgent) {Model-generated};
      \node[legendbox, draw=purple!70!black, fill=purple!12, right=2mm of lgent] (l1) {};
      \node[right=0.6mm of l1, font=\tiny] (l1t) {Special tokens};
      \node[legendbox, draw=orange!80!black, fill=orange!22, right=2mm of l1t] (l3) {};
      \node[right=0.6mm of l3, font=\tiny] {KB value};
    }%
  };

\end{tikzpicture}


==> figures/KARLA_tokens_fabian.tex <==
\begin{figure}
\setstcolor{red}
A. Fine-tuning corpus {\small (generated from KB)}
\begin{framed}
Paris is the capital of $\langle$isCapOf$\rangle$.\\
Paris has $\langle$numHab$\rangle$ inhabitants.\\
... 
\end{framed}

B. Output {\small (generated by KARLA)}
\begin{framed}
London has \st{$\langle$numHab$\rangle$} inhabitants.\\
\textcolor{white}{London has }\textcolor{red}{9,089,736} {\small (pulled in from KB)}
\end{framed}
\caption{KARLA in action \fms{adding this in here again for comparison: It showed both the training and the inference, and was rather sober in layout...}}
\label{fig:tokens2}
\end{figure}


==> figures/main_figure_tikz.tex <==
% =====================================================================
% Self-contained color setup (safe when \input'd from anywhere)
% =====================================================================
\makeatletter
\@ifundefined{color@kbpurple}{\definecolor{kbpurple}{HTML}{534AB7}}{}
\@ifundefined{color@teacheramber}{\definecolor{teacheramber}{HTML}{BA7517}}{}
\@ifundefined{color@panelborder}{\definecolor{panelborder}{HTML}{B4B2A9}}{}
\@ifundefined{color@neutralgray}{\definecolor{neutralgray}{HTML}{6F6F6F}}{}
\@ifundefined{color@frameA}{\definecolor{frameA}{HTML}{F4EFE3}}{}
\@ifundefined{color@frameB}{\definecolor{frameB}{HTML}{ECEEF4}}{}
\@ifundefined{color@kbpurplelight}{\definecolor{kbpurplelight}{HTML}{EDEBF8}}{}
\@ifundefined{color@amberlight}{\definecolor{amberlight}{HTML}{F8EFDC}}{}
\@ifundefined{color@annotgreen}{\definecolor{annotgreen}{HTML}{0F6E56}}{}
\@ifundefined{color@annotgreenlight}{\definecolor{annotgreenlight}{HTML}{E3F1EB}}{}
\@ifundefined{color@relationred}{\definecolor{relationred}{HTML}{993556}}{}
\@ifundefined{color@kbblue}{\definecolor{kbblue}{HTML}{185FA5}}{}
\@ifundefined{color@missred}{\definecolor{missred}{HTML}{A32D2D}}{}
\@ifundefined{color@missredlight}{\definecolor{missredlight}{HTML}{F8E5E5}}{}
\@ifundefined{color@inputgray}{\definecolor{inputgray}{HTML}{E8E7E1}}{}
\@ifundefined{color@inputborder}{\definecolor{inputborder}{HTML}{8E8D86}}{}
\@ifundefined{color@arrowgray}{\definecolor{arrowgray}{HTML}{6F6F6F}}{}
\makeatother

\begin{figure*}[t]
\centering
\begin{tikzpicture}[
  font=\footnotesize,
  >={Stealth[length=2mm,width=1.5mm]},
  arrow/.style={->, draw=arrowgray, line width=0.5pt},
  dasharrow/.style={->, draw=arrowgray, line width=0.5pt, dashed},
  kbblock/.style={rectangle, rounded corners=2pt, draw=kbpurple, line width=0.4pt, fill=kbpurplelight, inner sep=2pt, align=center},
  teacherblock/.style={rectangle, rounded corners=2pt, draw=teacheramber, line width=0.4pt, fill=amberlight, inner sep=2pt, align=center},
  annotblock/.style={rectangle, rounded corners=2pt, draw=annotgreen, line width=0.4pt, fill=annotgreenlight, inner sep=2pt, align=center},
  llmblock/.style={rectangle, rounded corners=2pt, draw=relationred, line width=0.4pt, fill=missredlight!40!white, inner sep=2pt, align=center},
  ioblock/.style={rectangle, rounded corners=2pt, draw=inputborder, line width=0.4pt, fill=inputgray, inner sep=2pt, align=center},
  outgrounded/.style={rectangle, rounded corners=2pt, draw=annotgreen, line width=0.4pt, fill=annotgreenlight, inner sep=2pt, align=center},
  outfallback/.style={rectangle, rounded corners=2pt, draw=missred, line width=0.4pt, fill=missredlight, inner sep=2pt, align=center},
  diamondblock/.style={diamond, aspect=2, draw=teacheramber, line width=0.4pt, fill=amberlight, inner sep=0pt, align=center},
  panelA/.style={rectangle, rounded corners=3pt, draw=panelborder, line width=0.4pt, fill=frameA},
  panelB/.style={rectangle, rounded corners=3pt, draw=panelborder, line width=0.4pt, fill=frameB},
]

% ============== PANEL A: TRAINING (one row, 4 equal blocks) ==============
\node[kbblock, minimum width=38mm, minimum height=36mm] (kbbox) at (0,0) {};
\node[anchor=north, align=center, yshift=-1.5mm, font=\fontfamily{phv}\selectfont] at (kbbox.north)
  {\textbf{\textcolor{kbpurple}{1.\ KB sampling}}\\\textcolor{kbpurple!85!black}{\scriptsize Entity subgraph}};
\begin{scope}[shift={($(kbbox.center)+(0,-2mm)$)}, scale=0.85, transform shape]
  \coordinate (center) at (0,0);
  \coordinate (n1) at (-0.95,0.55);  \coordinate (n2) at (0.95,0.55);
  \coordinate (n3) at (-0.95,-0.5);  \coordinate (n4) at (0.95,-0.5);
  \draw[kbpurple, line width=0.3pt] (center) -- (n1);
  \draw[kbpurple, line width=0.3pt] (center) -- (n2);
  \draw[kbpurple, line width=0.3pt] (center) -- (n3);
  \draw[kbpurple, line width=0.3pt] (center) -- (n4);
  \filldraw[kbpurple] (center) circle (3.2mm);
  \node[white, font=\fontfamily{phv}\selectfont\bfseries\tiny] at (center) {France};
  \filldraw[kbpurple!50] (n1) circle (1.7mm);
  \filldraw[kbpurple!50] (n2) circle (1.7mm);
  \filldraw[kbpurple!50] (n3) circle (1.7mm);
  \filldraw[kbpurple!50] (n4) circle (1.7mm);
  \node[font=\fontfamily{phv}\selectfont\tiny, above=-1pt of n1] {Paris};
  \node[font=\fontfamily{phv}\selectfont\tiny, above=-1pt of n2] {60M};
  \node[font=\fontfamily{phv}\selectfont\tiny, below=-1pt of n3] {EUR};
  \node[font=\fontfamily{phv}\selectfont\tiny, below=-1pt of n4] {EU};
\end{scope}
\node[anchor=south, font=\fontfamily{phv}\selectfont\tiny, align=center, yshift=1pt] at (kbbox.south)
  {Triples $(s,r,o)$:\ (France, capital, Paris)};

\node[teacherblock, minimum width=38mm, minimum height=36mm,
      right=5mm of kbbox.east, font=\fontfamily{phv}\selectfont] (teacher)
  {\textbf{\textcolor{teacheramber}{2.\ Teacher LLM}}\\[1pt]\textcolor{teacheramber!85!black}{\scriptsize Annotates with tags}\\[6pt]\textcolor{teacheramber!85!black}{\scriptsize retry $\leq R$ if invalid}};
\draw[teacheramber, line width=0.4pt, ->]
  ([yshift=3mm,xshift=-3mm]teacher.east) .. controls +(7mm,2mm) and +(7mm,-2mm) .. ([yshift=-3mm,xshift=-3mm]teacher.east);

\node[annotblock, minimum width=38mm, minimum height=36mm,
      right=5mm of teacher.east] (annot) {};
\node[anchor=north, align=center, yshift=-1.5mm,
      font=\fontfamily{phv}\selectfont\bfseries] at (annot.north)
  {\textcolor{annotgreen}{Annotated text}};
\node[anchor=center, font=\fontfamily{phv}\selectfont\scriptsize,
      align=left, text=neutralgray, yshift=-2mm] at (annot.center)
{\textquotedblleft Paris is the capital of\\
\textcolor{relationred}{$\langle$capital$\rangle$}\textcolor{annotgreen}{$\langle$subj$\rangle$}France\textcolor{annotgreen}{$\langle$/subj$\rangle$}\\
\textcolor{relationred}{$\langle$/capital$\rangle$}, which lies\\
on the Seine\dots\textquotedblright};

\node[llmblock, minimum width=38mm, minimum height=36mm,
      right=5mm of annot.east] (kbllm) {};
\node[anchor=north, align=center, yshift=-1.5mm,
      font=\fontfamily{phv}\selectfont] at (kbllm.north)
  {\textbf{\textcolor{relationred}{3.\ KB-LLM}}\\\textcolor{relationred!85!black}{\scriptsize Fine-tuned on corpus}};
\node[anchor=south, font=\fontfamily{phv}\selectfont\scriptsize,
      text=relationred!85!black, align=center, yshift=2mm] at (kbllm.south)
{Loss masked on\\$\langle$KB$\rangle$\,\dots\,$\langle$/KB$\rangle$ spans};

\draw[arrow] (kbbox.east) -- (teacher.west);
\draw[arrow] (teacher.east) -- (annot.west);
\draw[arrow] (annot.east) -- (kbllm.west);

\node[anchor=south west, align=left, inner sep=0pt]
  at ($(kbbox.north west)+(0,2mm)$)
  {\fontfamily{phv}\selectfont\textbf{\footnotesize\textcolor{neutralgray}{A.\ Training}}%
   \hspace{2mm}\fontfamily{phv}\selectfont\scriptsize\textcolor{neutralgray}{Build annotated synthetic corpus, then fine-tune with masked loss on KB spans}};

\begin{pgfonlayer}{background}
  \node[panelA, fit=(kbbox)(teacher)(annot)(kbllm), inner sep=4mm, yshift=-1mm] (panelABG) {};
\end{pgfonlayer}

% ============== PANEL B: INFERENCE (two rows, 4 equal blocks each) ==============
\node[ioblock, minimum width=38mm, minimum height=14mm,
      below=10mm of panelABG.south west, anchor=north west,
      font=\fontfamily{phv}\selectfont] (input)
  {\textbf{Input}\\\textcolor{neutralgray}{\scriptsize\textquotedblleft The capital of France is\dots\textquotedblright}};

\node[llmblock, minimum width=38mm, minimum height=14mm,
      right=5mm of input, font=\fontfamily{phv}\selectfont] (kbllmI)
  {\textbf{\textcolor{relationred}{KB-LLM}}\\\textcolor{relationred!85!black}{\scriptsize Generates tag}};

\node[annotblock, minimum width=38mm, minimum height=14mm,
      right=5mm of kbllmI] (tag)
  {\fontfamily{phv}\selectfont\scriptsize\textcolor{annotgreen}{$\langle$capital$\rangle$$\langle$subj$\rangle$France$\langle$/subj$\rangle$$\langle$/capital$\rangle$}};

\node[diamondblock, minimum width=38mm, minimum height=14mm,
      right=5mm of tag, font=\fontfamily{phv}\selectfont] (lookup)
  {\textbf{\textcolor{teacheramber}{KB lookup}}\\\textcolor{teacheramber!85!black}{\scriptsize(capital, France)}};

\node[outgrounded, minimum width=38mm, minimum height=14mm,
      below=10mm of input, font=\fontfamily{phv}\selectfont] (hitOut)
  {\textbf{\textcolor{annotgreen}{Output (grounded)}}\\\textcolor{neutralgray}{\scriptsize\textquotedblleft\dots is \textcolor{annotgreen}{\textbf{Paris}}, the capital of France.\textquotedblright}};

\node[outgrounded, minimum width=38mm, minimum height=14mm,
      right=5mm of hitOut] (hitContent)
  {\fontfamily{phv}\selectfont\scriptsize\textcolor{annotgreen}{$\langle$KB$\rangle$Paris\,:\,city$\langle$/KB$\rangle$}\\\fontfamily{phv}\selectfont\tiny\textcolor{annotgreen!85!black}{(retrieved from KB)}};

\node[outfallback, minimum width=38mm, minimum height=14mm,
      right=5mm of hitContent] (missContent)
  {\fontfamily{phv}\selectfont\scriptsize\textcolor{missred}{$\langle$KB\_FAIL$\rangle$}\\\fontfamily{phv}\selectfont\tiny\textcolor{missred!85!black}{(no KB grounding)}};

\node[outfallback, minimum width=38mm, minimum height=14mm,
      right=5mm of missContent, font=\fontfamily{phv}\selectfont] (missOut)
  {\textbf{\textcolor{missred}{Output (fallback)}}\\\textcolor{neutralgray}{\scriptsize\textquotedblleft\dots is \textcolor{missred}{\textbf{Paris}}, model's parametric guess.\textquotedblright}};

\draw[arrow] (input.east)   -- (kbllmI.west);
\draw[arrow] (kbllmI.east)  -- (tag.west);
\draw[arrow] (tag.east)     -- (lookup.west);

\draw[arrow] (lookup.south) -- ++(0,-5mm) -| (hitContent.north);
\node[font=\fontfamily{phv}\selectfont\bfseries\scriptsize, text=annotgreen,
      fill=frameB, inner sep=1pt]
  at ($(hitContent.north)+(15mm,2.5mm)$) {hit};

\draw[arrow] (lookup.south) -- ++(0,-5mm) -| (missContent.north);
\node[font=\fontfamily{phv}\selectfont\bfseries\scriptsize, text=missred,
      fill=frameB, inner sep=1pt]
  at ($(missContent.north)+(-15mm,2.5mm)$) {miss};

\draw[arrow] (hitContent.west) -- (hitOut.east);
\draw[arrow] (missContent.east) -- (missOut.west);

\node[anchor=south west, align=left, inner sep=0pt]
  at ($(input.north west)+(0,2mm)$)
  {\fontfamily{phv}\selectfont\textbf{\footnotesize\textcolor{neutralgray}{B.\ Inference}}%
   \hspace{2mm}\fontfamily{phv}\selectfont\scriptsize\textcolor{neutralgray}{KB-LLM emits a subject tag, KB is queried; output is grounded on hit, falls back on miss}};

% Dashed reference between Panel A's KB-LLM and Panel B's KB lookup
\draw[dasharrow, draw=panelborder]
  (kbllm.south) -- ($(kbllm.south)+(0,-3mm)$) -| (lookup.north);
\node[font=\fontfamily{phv}\selectfont\tiny, text=neutralgray, fill=white, inner sep=1pt]
  at ($(kbllm.south)!0.5!(lookup.north)$) {queries KB};

\begin{pgfonlayer}{background}
  \node[panelB, fit=(input)(kbllmI)(tag)(lookup)(hitOut)(hitContent)(missOut)(missContent),
        inner sep=4mm, yshift=-1mm] (panelBBG) {};
\end{pgfonlayer}

\node[draw=panelborder, rounded corners=2pt, line width=0.4pt,
      below=2mm of panelBBG.south, anchor=north,
      inner sep=4pt, fill=white, align=center]
  {\fontfamily{phv}\selectfont\scriptsize
   \textbf{Tag schema:}\quad
   \textcolor{annotgreen}{\textbf{$\langle$subj$\rangle$\dots$\langle$/subj$\rangle$}} subject entity\quad
   \textcolor{relationred}{\textbf{$\langle$relation$\rangle$\dots$\langle$/relation$\rangle$}} relation type\quad
   \textcolor{kbblue}{\textbf{$\langle$KB$\rangle$\dots$\langle$/KB$\rangle$}} KB span.\quad
   Loss is masked on $\langle$KB$\rangle$ spans during training.};

\end{tikzpicture}
\caption{KARLA methodology overview. \textbf{(A)} Training: triples sampled from a knowledge base are used by a teacher LLM to produce annotated synthetic text, on which KB-LLM is fine-tuned with the loss masked on KB spans. \textbf{(B)} Inference: KB-LLM emits a subject/relation tag, the KB is queried; the output is grounded on a hit or falls back on a miss.}
\label{fig:karla-method}
\end{figure*}

==> sections/05_discussion.tex <==
\fms{We might not have space for this section}

\paragraph{Externalization reallocates, rather than removes, the role of parametric knowledge.} \fms{Great ideas, which could go to the conclusion} A central finding of this work is that moving factual values out of the parameters does not collapse the model into a passive retrieval interface. Effective generation still requires identifying which entities to query, selecting appropriate relations, and integrating retrieved facts into coherent discourse. The gains from adding lightweight entity descriptions on PopQA and FActScore (Section 4.4) make this concrete: even when the KB supplies atomic values, a small amount of semantic context measurably helps the model plan useful lookups. We read this as a productive division of labor, parametric capacity is reallocated from rote factual storage toward interpretation and control, and as evidence that retrieval-path supervision and semantic competence are complementary rather than competing objectives.

\paragraph{Verifiability.} Because KARLA-trained models emit explicit retrieval paths and delimits KB-returned spans, every factual mention in a generation is traceable to a triple or to an explicit parametric fallback. This makes provenance inspectable at the token level and gives factual edits well-defined semantics: revising a triple changes downstream generation immediately, without retraining or weight editing (Section 4.3). We view this inspectability as a main practical contribution of the framework. \fms{to be a main contribution, we would have to highlight and evaluate it more. Better move to a demo paper.} \nils{Agreed for the demo paper. For this paper, perhaps we can frame this as "towards KB-supported verifiability"? For space, it is indeed possible to move the two ideas from the discussion into the conclusion. }

